The Value of Information: A Puzzle

We show that the total value of information to informed traders can be measured by the covariation between price changes and order flow. This covariation captures noise trader losses, which equal informed trader gains when market making is competitive. We estimate the value of information using high frequency data on US equities at $3.5 million per year. The aggregate value of information is 0.04% of market cap, considerably lower than the 0.67% in fees investors pay searching for superior returns according to French (2008), which we extend through 2024. We discuss potential resolutions for these puzzling findings.

==> tables/summarystats_aflam_f1_dCLNV_vvof_m5_t0_i1_200309_202412.tex <==
\begin{tabular*}{1\columnwidth}{@{\hskip\tabcolsep\extracolsep\fill}l*{8}{r}}
\toprule 
 \multicolumn{1}{l}{variable} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Std} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{q25} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{q75} & \multicolumn{1}{c}{Max} & \multicolumn{1}{c}{Obs} \\ 
\midrule 
 Information value (dPdY), \$M &  3.47~ &  61.58~ &  -1.11~ &  0.30~ &  1.02~ &  3.08~ &  52.30~ & 14,382,920 \\ 
 Information value ($\lambda \sigma_y^2$), \$M &  3.45~ &  61.73~ &  -1.11~ &  0.30~ &  1.01~ &  3.06~ &  52.15~ & 14,382,920 \\ 
 Orderflow Volatility, \$M &  45.03~ &  98.61~ &  0.07~ &  2.64~ &  10.36~ &  38.74~ &  662.18~ & 14,382,920 \\ 
 Price impact per \$M &  0.11~ &  0.38~ &  -0.06~ &  0.00~ &  0.01~ &  0.05~ &  2.92~ & 14,382,920 \\ 
 Stock price &  56.49~ &  152.30~ &  5.00~ &  17.84~ &  34.18~ &  62.75~ &  305,971.48~ & 14,382,920 \\ 
 Size (lnME) &  14.23~ &  1.82~ &  10.46~ &  12.92~ &  14.13~ &  15.41~ &  18.93~ & 14,382,920 \\ 
 Book-to-market ratio &  0.60~ &  0.45~ &  0.03~ &  0.28~ &  0.50~ &  0.80~ &  2.59~ & 14,382,920 \\ 
 Momentum &  0.18~ &  0.49~ &  -0.66~ &  -0.11~ &  0.10~ &  0.34~ &  2.50~ & 14,382,920 \\ 
 Earnings &  0.01~ &  0.11~ &  0.00~ &  0.00~ &  0.00~ &  0.00~ &  1.00~ & 14,382,920 \\ 
\bottomrule 
\end{tabular*} 

